On Coresets for Clustering in Small Dimensional Euclidean Spaces

We consider the problem of constructing small coresets for $k$-Median in Euclidean spaces. Given a large set of data points $P\subset \mathbb{R}^d$, a coreset is a much smaller set $S\subset \mathbb{R}^d$, so that the $k$-Median costs of any $k$ centers w.r.t. $P$ and $S$ are close. Existing literature mainly focuses on the high-dimension case and there has been great success in obtaining dimension-independent bounds, whereas the case for small $d$ is largely unexplored. Considering many applications of Euclidean clustering algorithms are in small dimensions and the lack of systematic studies in the current literature, this paper investigates coresets for $k$-Median in small dimensions. For small $d$, a natural question is whether existing near-optimal dimension-independent bounds can be significantly improved. We provide affirmative answers to this question for a range of parameters. Moreover, new lower bound results are also proved, which are the highest for small $d$. In particular, we completely settle the coreset size bound for $1$-d $k$-Median (up to log factors). Interestingly, our results imply a strong separation between $1$-d $1$-Median and $1$-d $2$-Median. As far as we know, this is the first such separation between $k=1$ and $k=2$ in any dimension.

==> d2k2.tex <==
\section{Improved Coreset Lower Bound in $\R^d$ when $k\geq 2$}\label{sec:lb}

We present a lower bound for the coreset size in small dimensional spaces. 

\begin{theorem}[\bf{Coreset lower bound in small dimensional spaces}]
\label{thm:lowerbound_appendix}
Given an integer $k$ and a real number $\epsilon \in (0,1)$, for any integer $d \le \frac{1}{45} \frac{1}{\epsilon^2}$, there is a data set $P \subset \R^{d+1}$ such that its $\epsilon$-coreset must contain at least $\frac{1}{10} dk$ points.
\end{theorem}

\noindent
When $d = \Theta(\frac{1}{\epsilon^2})$, Theorem~\ref{thm:lowerbound_appendix} gives the well known lower bound $\frac{k}{\epsilon^2}$. When $d \ll \Theta(\frac{1}{\epsilon^2})$, the theorem is non-trivial.

\begin{proof}
We work on $\R^{d+1}$ instead of working on $\R^d$ for technical reasons. We will construct $k$ $d$-dimensional affine subspaces in $\R^{d+1}$, each of them is far away from others. Then we consider the standard basis in each subspace and show that a coreset of the data set must contain at least $\Omega(kd)$ points.

Denote the standard basis in $\R^{d+1}$ by $e_0,\dots,e_d$. For each $j \in [k]$, we consider the data set $P_j \triangleq jLe_0 + \{ e_1, e_2, \dots, e_d\}$ where $L$ is a positive number large enough. We take the full data set $P$ as $P = \cup_{j \in [k]} P_j$. Each $P_j$ lies in a $d$-dimensional affine subspace $jLe_0 + \text{span}\left<e_1,\dots,e_d\right>$. These affine subspaces are far away from each other since $L$ is large enough, and this separation property assures that we can analyze these affine subspaces independently.

Denote the coreset of $P$ as $C$. For each $j \in [k]$, denote $C_j \triangleq C \cap P_j$. If $jLe_0  + e_i \in C_j$, we denote $i \in C_j$ for the sake of convenience, we also denote its coreset weight as $w_i$. Denote $v_j \triangleq \sum_{i \in C_j} w_i e_i - \sum_{i=1}^d e_i$, we consider the query $Q = \{q_1,\dots,q_k\}$ where $q_j \triangleq \frac{v_j}{\| v_j\|_2} + jLe_0 $. 

Note that each $p \in P_j$ has $q_j$ as its closet query point since $L$ is large enough, thus $\cost(P,Q) = \sum_{j=1}^k \cost(P_j,Q) = \sum_{j=1}^k \cost(P_j,q_j)$ and  $\cost(C,Q) = \sum_{j=1}^k \cost(C_j,q_j)$. We compute $\cost(P,Q)$ and $\cost(C,Q)$ by computing $\cost(P_j,q_j)$ and $\cost(C_j,q_j)$

We compute $\cost(P_j,q_j)$ first, that is 
\begin{align*}
    \cost(P_j,q_j) &= \sum_{i=1}^d \|jLe_0 + e_i - q_j\|^2=   \sum_{i=1}^d \| e_i - \frac{v_j}{|v_j|}\|^2= 2d - 2\sum_{i=1}^d \left< e_i,\frac{v_j}{|v_j|}\right>.
\end{align*}

Similarly we have $\cost(C_j,q_j) =  2\sum_{i \in C_j} w_i - 2\sum_{i \in C_j} w_i \left< e_i,\frac{v_j}{|v_j|}\right>$. 

Combining them all, we have
\begin{align*}
 \quad \cost(P,Q) - \cost(C,Q) 
  = & \quad 2kd - 2\sum_{j=1}^k \sum_{i \in C_j} w_i + 2 \sum_{j=1}^k \left< \sum_{i \in C_j} w_i e_i - \sum_{i=1}^d e_i, \frac{v_j}{|v_j|}\right>\\
  = & \quad 2kd - 2\sum_{j=1}^k \sum_{i \in C_j} w_i + 2 \sum_{j=1}^k \| v_j\|.
\end{align*}

The coreset property implies that $|\cost(P,Q) - \cost(C,Q)| \le \epsilon \cost(P,Q) \le 4\epsilon kd$, thus we have 
\begin{equation}
\label{inequality:coreset_property}
    2kd - 2\sum_{j=1}^k \sum_{i \in C_j} w_i + 2 \sum_{j=1}^k \| v_j\| \le 4\epsilon kd.
\end{equation}


Taking $\tilde{Q} = \{Le_0,2Le_0,3Le_0,\dots,kLe_0\}$, we have $\cost(P,\tilde{Q}) = kd$ and $\cost(C,\tilde{Q}) = \sum_{j=1}^K \sum_{i \in C_j} w_i$, the coreset property then gives that $|kd - \sum_{j=1}^K \sum_{i \in C_j} w_i| \le \epsilon kd$. Substitute this inequality to inequality~\ref{inequality:coreset_property}, we get
\begin{equation}
\label{inequality:sum_of_query_norm}
    \sum_{j=1}^k \| v_j\| \le 3\epsilon kd.
\end{equation}

For each $j \in [k]$, we have that $\|v_j\| = \| \sum_{i \in C_j} w_i e_i - \sum_{i=1}^d e_i\| \ge \| \sum_{i \not \in C_j} e_i\| = \sqrt{\#(P_j) - \#(C_j)}$. Substitute this inequality to inequality~\ref{inequality:sum_of_query_norm}, we have 
\begin{equation}
    \label{inequality:coreset_size}
    \sum_{j=1}^k \sqrt{\#( P_j) - \#(C_j)} \le 3\epsilon kd.
\end{equation}

Our goal is to show that $\#(C) \ge \frac{1}{10} kd = \frac{1}{10} \#(P)$, we prove it by contradiction. We will show that if $\#(C) \ge \frac{1}{10} \#(P)$ then the dimension $d$ is larger than $\frac{1}{45} \frac{1}{\epsilon^2}$, which contradicts to the assumption on $d$.

Assume that $\#(C) \le \frac{1}{10} \#(P) = \frac{1}{10} kd$, then for at least half of $P_j$ we have $\#(C_j) \le \frac{1}{5} \#(P_j)$ and thus $\#( P_j) - \#(C_j) \ge \frac{4}{5} \#(P_j) = \frac{4}{5}d$. Summing over these $P_j$ we have $\sum_{j=1}^k \sqrt{\#( P_j) - \#(C_j)} \ge \frac{k}{2} \sqrt{\frac{4}{5}d} =  k \sqrt{\frac{1}{5} d}$. By inequality~\ref{inequality:coreset_size} we have $k \sqrt{\frac{1}{5}d} \le 3 \epsilon k d$, thus $\frac{1}{45} \frac{1}{\epsilon^2} \le d$. This leads to a contradiction.
\end{proof}

\begin{remark}
The proof assumes that the coreset is a subset of the original data set, and the proof holds for coreset with offset.
\end{remark}

\section{Generalized lower bound for \kMeans clustering with general $S$.}
The lower bound proved above relies on the assumption that the coreset $S$ is a subset of the original dataset. Next we generalize the result by allowing arbitrary $S$ in $\R^{d+1}$. 

\subsection{Preparation}
\paragraph{Additional notation} Let $e_0, \cdots, e_d$ be the standard basis vectors of $\R^{d+1}$, and $H_1,\cdots,H_{k/2}$ be $k/2$ $d$-dimensional affine subspaces, where $H_j := jLe_0 + \text{span}\left\{e_1,\dots,e_d\right\}$ for a sufficiently large constant $L$. For any $p\in \R^{d+1}$, we use $\Tilde{p}$ to denote the $d$-dimensional vector $p_{1:d}$ (i.e., discard the $0$-th coordinate of $p$).

\paragraph{Hard instance} The hard instance is the same as in Section~\ref{sec:lb}, except that now there are $k/2$ affine subspaces and in each affine subspace $H_j$, we only put $d/2$ points, which are $jLe_0+e_1,\cdots, jLe_0+e_{d/2}$. Similarly, we use $P_j$ to denote the data points in $H_j$ ($j=1,\cdots,k/2$) and let $P$ be the union of all $P_j$. Thus, $|P|=kd/4$. In our proof, we always put two centers in each $H_j$; for large enough $L$, all $p\in P_j$ must be assigned to centers in $H_j$.

We will use the following two technical lemmas from \citep{cohenaddad2022towards}.
\begin{lemma}\label{lem:cost-to-basis}
For any $k\ge 1$, let $\{c_1,\cdots,c_k\}$ be arbitrary $k$ unit vectors in $\R^d$, we have
\begin{align*}
    \sum_{i=1}^{d/2} \min_{\ell=1}^k\|e_i-c_{\ell}\|^2 \ge d-\sqrt{dk/2}.
\end{align*}
\end{lemma}
\begin{lemma}\label{lem:cost-to-smallset}
Let $S$ be a set of points in $\R^d$ of size $t$ and $w: S\rightarrow \R^+$ be their weights. There exist $2$ unit vectors $v_1, v_2$, such that
\begin{align*}
    \sum_{p\in S} w(p)\min_{\ell=1,2} \|p-v_{\ell}\|^2 \le \sum_{s\in P}w(p)(\|p\|^2+1)-  \frac{2\sum_{p\in S} w(p)\|p\|}{\sqrt{t}}.
\end{align*}
\end{lemma}

\subsection{Proof of the Lower Bound}
\noindent
Next, we present the lower bound result and its proof.
\begin{theorem}[\bf{Same coreset lower bound when $S$ can be arbitrary}]
\label{thm:lowerbound-general}
Given an integer $k$, a real number $\epsilon \in (0,1)$, and integer $d \le \frac{1}{100\epsilon^2}$, let $P \subset \R^{d+1}$ be the point set described above. For any $S\subset \R^{d+1}$, if it is a $\eps$-coreset of $P$, then we must have $|S|=\Omega(dk)$.
\end{theorem}
\begin{proof}
Note that points in $S$ might not be in any $H_j$. We first map each point $p\in S$ to an index $j_p\in [k/2]$ such that $H_{j_p}$ is the nearest subspace of $p$. The mapping is quite simple: 
\begin{align*}
    j_p = \arg\min_{j\in[k/2]} |p_0 - jL|,
\end{align*}
where $p_0$ is the $0$-th coordinate of $p$.
Let $\Delta_p = p_0 - j_pL$, which is the distance of $p$ to the closest affine subspace. Let $S_j:=\{p\in S: j_p=j\}$ be the set of points in $P$, whose closest affine subspace is $H_j$. Define $I:=\{j\in[k/2] : |S_j| \le d/4\}$. Consider any $k$-center set $C$ such that $H_j\bigcap C \neq \emptyset$. Then $\cost(P, C)\ll 0.1 L$ for sufficiently large $L$. On the other hand, $\cost(S, C) \ge \sum_{p\in S} \Delta_p^2$. Since $S$ is a coreset, $\Delta_p^2 \ll L$ for all $p\in S$. \footnote{Here we do not allow offsets to simplify the proof, but our technique can be extended to handle offsets.} Therefore each $p\in S$ must be very close to its closest affine subspace; in particular, we can assume that $p$ must be assigned to some center in $H_{j_p}$ (if there exists one).

In the proof follows, we consider three different set of $k$ centers $C_1,C_2$ and $C_3$ and compare the costs $\cost(P, C_i)$ and $\cost(S, C_i)$ for $i=1,2,3$. In each $C_i$, there are two centers in each $H_j$. As we have discussed above, for large enough $L$, the total cost for both $P$ and $S$ can be decomposed into the sum of costs over all affine subspaces.

For each $j\in \Bar{I}$, the corresponding centers in $H_j$ are the same across $C_1,C_2,C_3$. Let $c_j$ be any point in $H_j$ such that $c_j-jLe_0$ has unit norm and is orthogonal to $e_1,\cdots,e_{d/2}$; in other words, $\|\Tilde{c}_j\|=1$ and the first $d/2$ coordinates of $\Tilde{c}_j=1$ are all zero. Specifically, we set $c_j = jLe_0 + e_{d/2+1}$ and the two centers in $H_j$ are two copies of $c_j$ for $j\in \Bar{I}$. 

We first consider the following $k$ centers denoted by $C_1$. As we have specified the centers for $j\in \Bar{I}$, we only describe the centers for each $j\in I$. Since by definition, $|S_j|\le d/4$, we can find a vector $c_j\in \R^{d+1}$ in $H_j$ such that $c_j-jLe_0$ has unit norm and is orthogonal to $e_1,\cdots,e_{d/2}$ and all vectors in $S_j$. Let $C_1$ be the set of $k$ points with each point in $\{c_1,\cdots,c_{k/2}\}$ copied twice. We evaluate the cost of $C_1$ with respect to $P$ and $S$. 
\begin{lemma}
    For $C_1$ constructed above, we have $\cost(P,C_1) = \frac{kd}{2}$ and 
    \begin{align*}
        \cost(S,C_1) =\sum_{p\in S} w(p)(\Delta_p^2+\|\Tilde{p}\|^2 +1) - 2\sum_{j\in \Bar{I}}\sum_{p\in S_j}w(p)\langle p-jLe_0, jLe_0-c_j \rangle.
    \end{align*}
\end{lemma}
\begin{proof}
Since $e_i$ is orthogonal to $c_j-jLe_0$ and $c_j-jLe_0$ has unit norm for all $i,j$, it follows that
\begin{align}
\cost(P,C_1) &=
    \sum_{j=1}^{k/2}\sum_{i=1}^{d/2} \min_{c\in C_1}\|jLe_0+e_i-c\|^2 = \sum_{j=1}^{k/2} \sum_{i=1}^{d/2} \|jLe_0+e_i -c_j\|^2 \nonumber\\
    &=\sum_{j=1}^{k/2}\sum_{i=1}^{d/2}(\|e_i\|^2+\|c_j-jLe_0\|^2-2\langle e_i, c_j-jLe_0 \rangle )\nonumber\\
    &=\frac{kd}{2}.\label{eqn:cost-of-c}
\end{align}
On the other hand, the cost of $C$ w.r.t.\ $S_j$ is
\begin{align}
    \sum_{p\in S_j} \min_{c\in C_1}w(p)\|p-c\|^2 &= \sum_{p\in S_j} w(p)\|p-c_j\|^2 = \sum_{p\in S_j} w(p)\|p-jLe_0+ jLe_0-c_j\|^2 \nonumber\\
    &= \sum_{p\in S_j}w(p)\left(\|p-jLe_0\|^2 + 1 -2\langle p-jLe_0, jLe_0-c_j \rangle \right)\nonumber\\
    &= \sum_{p\in S_j} w(p)(\Delta_p^2+\|\Tilde{p}\|^2 +1) -2w(p)\langle p-jLe_0, jLe_0-c_j \rangle .\label{eqn:cost-of-c-to-S}
\end{align}
Recall $\Tilde{p}\in \R^d$ is $p_{1:d}$. 
For $j\in I$, the inner product is $0$, and thus the total cost w.r.t.\ $S$ is 
\begin{align*}
    \cost(S,C_1) = \sum_{p\in S} w(p)(\Delta_p^2+\|\Tilde{p}\|^2 +1) - 2\sum_{j\in \Bar{I}}\sum_{p\in S_j}w(p)\langle p-jLe_0, jLe_0-c_j \rangle,
\end{align*}
which finishes the proof.
\end{proof}

For notational convenience, we define $\kappa := 2\sum_{j\in \Bar{I}}\sum_{p\in S_j}w(p)\langle p-jLe_0, jLe_0-c_j \rangle$.
Since $S$ is an $\eps$-coreset of $P$, we have 
\begin{align}\label{eqn:weight-constraints}
    dk/2- \eps dk/2\le \sum_{p\in S} w(p)(\Delta_p^2+\|p'\|^2 +1) - \kappa \le dk/2+\eps dk/2.
\end{align}

Next we consider a different set of $k$ centers denoted by $C_2$. By Lemma~\ref{lem:cost-to-smallset}, there exists unit vectors $v^j_1,v^j_2 \in \R^d$ such that
\begin{align}
    \sum_{p\in S_j} w(p)(\min_{\ell=1,2} \|\Tilde{p}-v^j_{\ell}\|^2+\Delta_p^2) \le \sum_{p\in S_j}w(p)(\|\Tilde{p}\|^2+1 + \Delta_p^2)-  \frac{2\sum_{p\in S_j} w(p)\|\Tilde{p}\|}{\sqrt{|S_j|}}. \label{eqn:small-coreset-cost}
\end{align}
Applying this to all $j\in I$ and get corresponding $v^j_1,v^j_2$ for all $j\in I$. Let $C_2=\{u_1^1,u_2^2,\cdots, u_1^{k/2},u_2^{k/2}\}$ be a set of $k$ centers in $\R^{d+1}$ defined as follows: if $j\in I$, $u_{\ell}^j$ is $v_{\ell}^j$ with an additional $0$th coordinate with value $jL$, making them lie in $H_j$; for $j\in \Bar{I}$, we use the same centers as in $C_1$, i.e., $u_{1}^j=u_{2}^j =c_j$. 

\begin{lemma}
    For $C_2$ constructed above, we have 
    \begin{align*}
        \cost(P,C_2) \ge \frac{kd}{2}-\sqrt{d}|I| \text{ and } 
    \end{align*} 
    \begin{align*}
        \cost(S,C_2) \le \sum_{p\in S}w(p)(\|\Tilde{p}\|^2+1+\Delta_p^2)-  \sum_{j\in I} \frac{2\sum_{p\in S_j} w(p)\|\Tilde{p}\|}{\sqrt{|S_j|}} -\kappa.
    \end{align*}
\end{lemma}
\begin{proof}
By \eqref{eqn:small-coreset-cost}, 
\begin{align*}
\cost(S,C_2) &= \sum_{j=1}^{k/2} \sum_{p\in S_j}w(p)\min_{c\in C_2}\|p-c\|^2 =
    \sum_{j\in I}\sum_{p\in S_j} w(p)\min_{\ell=1,2} (\|\Tilde{p}-v^j_{\ell}\|^2+\Delta^2_p) +\sum_{j\in \Bar{I}} \sum_{p\in S_j}w(p)\|p-c_j\|^2\\
    &\le \sum_{p\in S}w(p)(\|\Tilde{p}\|^2+1+\Delta_p^2)-  \sum_{j\in I} \frac{2\sum_{p\in S_j} w(p)\|\Tilde{p}\|}{\sqrt{|S_j|}} -\kappa.
\end{align*}
By Lemma~\ref{lem:cost-to-basis} (with $k=2$), we have
\begin{align*}
    \sum_{i=1}^{d/2} \min_{\ell=1,2}\|e_i-v^j_{\ell}\|^2 \ge {d}-\sqrt{d}.
\end{align*}
It follows that
\begin{align*}
    \cost(P,C_2)&=\sum_{j=1}^{k/2}\sum_{i=1}^{d/2} \min_{c\in C_2}\|jLe_0+e_i-c\|^2 = \sum_{j\in I}\sum_{i=1}^{d/2} \min_{\ell=1,2} \|e_i-v^{j}_{\ell}\|^2 + \sum_{j\in \Bar{I}}\sum_{i=1}^{d/2} \|jLe_0+e_i-c\|^2 \\
    &\ge \frac{kd}{2}-\sqrt{d}|I|,
\end{align*}
where in the inequality, we also used the orthogonality between $e_i$ and $c_j-jLe_0$.
\end{proof}

Since $S$ is an $\eps$-coreset of $P$, we have
\begin{align*}
    \frac{dk}{2}-|I|\sqrt{d} - \frac{\eps dk}{2} \le (\frac{dk}{2}-|I|\sqrt{d})(1-\eps) \le \sum_{p\in S}w(p)(\|\Tilde{p}\|^2+1+\Delta_p^2)-  \sum_{j\in I} \frac{2\sum_{p\in S_j} w(p)\|\Tilde{p}\|}{\sqrt{|S_j|}}-\kappa,
\end{align*}
which implies
\begin{align}
    \sum_{j\in I} \frac{2\sum_{p\in S_j} w(p)\|\Tilde{p}\|}{\sqrt{|S_j|}}
    &\le \sum_{p\in S}w(p)(\|\Tilde{p}\|^2+1+\Delta_p^2) -\frac{dk-2|I|\sqrt{d}-\eps kd}{2}-\kappa
    \nonumber\\
    &\le  \frac{dk+\eps dk}{2} - \frac{dk-2|I|\sqrt{d}-\eps kd}{2} \quad\textnormal{by \eqref{eqn:weight-constraints}} \nonumber\\
    &= |I|\sqrt{d} +\eps kd. \nonumber
\end{align}
By definition, $|S_j| \le d/4$, so
\begin{align*}
      \sum_{j\in I} \frac{2\sum_{p\in S_j} w(p)\|\Tilde{p}\|}{\sqrt{d/4}}\le \sum_{j\in I} \frac{2\sum_{p\in S_j} w(p)\|\Tilde{p}\|}{\sqrt{|S_j|}},
\end{align*}
and it follows that
\begin{align}\label{eqn:size-constraint}
     \frac{\sum_{j\in I} \sum_{p\in S_j} w(p)\|\Tilde{p}\|}{\sqrt{d}} 
     \le \frac{|I|\sqrt{d} +\eps kd} {4}.
\end{align}

Finally we consider a third set of $k$ centers $C_3$. Similarly, there are two centers per group. We set $m$ be a power of $2$ in $[d/2,d]$. Let $h_1,\cdots,h_m$ be the $m$-dimensional Hadamard basis vectors. So all $h_{\ell}$'s are $\{-\frac{1}{\sqrt{m}},\frac{1}{\sqrt{m}}\}$ vectors and $h_1=(\frac{1}{\sqrt{m}},\cdots,\frac{1}{\sqrt{m}})$. We slightly abuse notation and treat each $h_{\ell}$ as a $d$-dimensional vector by concatenating zeros in the end. For each $h_{\ell}$ construct a set of $k$ centers as follows. For each $j\in \Bar{I}$, we still use two copies of $c_j$.  For $j\in I$, the $0$th coordinate of the two centers is $jL$, then we concatenate $h_{\ell}$ and $-h_{\ell}$ respectively to the first and the second centers. 
\begin{lemma}\label{lem:hadamard-cost}
     Suppose $C_3$ is constructed based on $h_{\ell}$. Then for all $\ell\in [m]$, we have 
    \begin{align*}
        \cost(P,C_3) = \frac{kd}{2} -\frac{d|I|}{\sqrt{m}}\text{ and } 
    \end{align*} 
    \begin{align*}
        \cost(S,C_3) = \sum_{p\in S} w(p) (\|\Tilde{p}\|^2+1 + \Delta_p^2) - 2\sum_{j\in I} \sum_{p\in S_j}\langle w(p) \Tilde{p}, h^p_{\ell} \rangle -\kappa.
    \end{align*}
\end{lemma}
\begin{proof}
For $j\in I$, the cost of the two centers w.r.t.\ $P_j$ is
\begin{align*}
    \cost(P_j,C_3) = \sum_{i=1}^{d/2} \min_{s=-1,+1}\|e_i - s\cdot h_{\ell}\|^2 = \sum_{i=1}^{d/2} (2-2\max_{s=-1,+1}\langle h_{\ell},e_i\rangle)=\sum_{i=1}^{d/2} (2-\frac{2}{\sqrt{m}}) = d-\frac{d}{\sqrt{m}}.
\end{align*}
For $j\in \Bar{I}$, the cost w.r.t.\ $P_j$ is $d$ by \eqref{eqn:cost-of-c}.
Thus, the total cost over all subspaces is 
\begin{align*}
\cost(P,C_3) =    (d-\frac{d}{\sqrt{m}})|I| + \left(\frac{k}{2} -|I| \right)d = \frac{kd}{2} -\frac{d|I|}{\sqrt{m}}.
\end{align*} 

On the other hand, for $j\in I$, the cost w.r.t.\ $S_j$ is 
\begin{align*}
    \sum_{p\in S_j} w(p)(\Delta_p^2+ \min_{s=\{-1,+1\}} \|\Tilde{p}-s\cdot h_{\ell}\|^2) &=\sum_{p\in S_j} w(p) (\|\Tilde{p}\|^2+1 + \Delta_p^2 - 2\max_{s=\{-1,+1\}}\langle \Tilde{p}, s\cdot h_{\ell} \rangle)\\
   & =\sum_{p\in S_j} w(p) (\|\Tilde{p}\|^2+1 + \Delta_p^2 - 2\langle \Tilde{p}, h^p_{\ell} \rangle).
\end{align*}
Here $h^p_{\ell} = s^p\cdot h_{\ell}$, where  $s^p=\arg\max_{s=\{-1,+1\}}\langle \Tilde{p}, s\cdot h_{\ell} \rangle$.
For $j\in \Bar{I}$, the cost w.r.t.\ $S_j$ is $\sum_{p\in S_j} w(p)(\Delta_p^2+\|\Tilde{p}\|^2 +1) -2\langle p-jLe_0, jLe_0-c_j \rangle )$ by \eqref{eqn:cost-of-c-to-S}. Thus, the total cost w.r.t.\ $S$ is
\begin{align*}
    \cost(S,C_3) = \sum_{p\in S} w(p) (\|\Tilde{p}\|^2+1 + \Delta_p^2) - 2\sum_{j\in I} \sum_{p\in S_j}\langle w(p) \Tilde{p}, h^p_{\ell} \rangle -\kappa .
\end{align*}
This finishes the proof.
\end{proof}

\begin{corollary}
Let $S$ be a $\eps$-coreset of $P$, and $I =\{j: |S_j|\le d/4\}$. Then 
\begin{align*}
    \sum_{j\in I}\sum_{p\in S_j} w(p)\|\Tilde{p}\| \ge \frac{d|I|-\eps kd\sqrt{d}}{2}. \\
\end{align*}
\end{corollary}
\begin{proof}
Since $S$ is an $\eps$-coreset, we have by Lemma~\ref{lem:hadamard-cost}
\begin{align*}
    2\sum_{j\in I} \sum_{p\in S_j}\langle w(p) \Tilde{p}, h^p_{\ell} \rangle &\ge \sum_{p\in S} w(p) (\|\Tilde{p}\|^2+1 + \Delta_p^2) -\kappa -(\frac{kd}{2} -\frac{d|I|}{\sqrt{m}})(1+\eps)\\
    &\ge \sum_{p\in S} w(p) (\|\Tilde{p}\|^2+1 + \Delta_p^2) -\kappa -\frac{kd}{2} +\frac{d|I|}{\sqrt{m}}-\frac{\eps kd}{2}\\
    &\ge \frac{dk-\eps dk}{2} - \frac{kd}{2} +\frac{d|I|}{\sqrt{m}}-\frac{\eps kd}{2} \quad\textnormal{by \eqref{eqn:weight-constraints}}\\
    &= \frac{d|I|}{\sqrt{m}} - \eps kd.
\end{align*}
Note that the above inequality holds for all $\ell\in[m]$, then 
$$ 2\sum_{\ell=1}^m\sum_{j\in I} \sum_{p\in S_j}\langle w(p) \Tilde{p}, h^p_{\ell}\rangle\ge d|I|\sqrt{m} - \eps kdm.$$

By the Cauchy-Schwartz inequality, 
\begin{align*}
    \sum_{\ell=1}^m\sum_{j\in I} \sum_{p\in S_j}\langle w(p) \Tilde{p}, h^p_{\ell} \rangle=  \sum_{j\in I}\sum_{p\in S_j}\langle w(p) \Tilde{p}, \sum_{\ell=1}^m h^p_{\ell} \rangle \le \sum_{j\in I}\sum_{p\in S_j} w(p)\|\Tilde{p}\| \|\sum_{\ell=1}^m h^p_{\ell} \| = \sqrt{m}\sum_{j\in I}\sum_{p\in S_j} w(p)\|\Tilde{p}\|.
\end{align*}
Therefore, we have
\begin{align*}
    \sum_{j\in I}\sum_{p\in S_j} w(p)\|\Tilde{p}\| \ge \frac{d|I|-\eps kd\sqrt{m}}{2} \ge \frac{d|I|-\eps kd\sqrt{d}}{2}.
\end{align*}
\end{proof}

Combining the above corollary with \eqref{eqn:size-constraint}, we have
\begin{align*}
    \frac{\sqrt{d}|I| -\eps kd }{2} \le \frac{|I|\sqrt{d} + \eps kd}{4} \implies |I| \le 3\eps k\sqrt{d}.
\end{align*}
By the assumption $d\le \frac{1}{100\eps^2}$, it holds that $|I| \le \frac{3k}{10}$ or $|\Bar{I}|\ge \frac{k}{2} -\frac{3k}{10}=\frac{k}{5}$. Moreover, since $|S_j|>\frac{d}{4}$ for each $j\in \Bar{I}$, we have $|S|>\frac{d}{4}\cdot \frac{k}{5} = \frac{kd}{20}$.
\end{proof}

\section{Lower Bound for Arbitrary $z$}
Using similar ideas from \citep{cohenaddad2022towards}, our proof of the lower bound for $z=2$ can be extended to arbitrary $z$. First, we provide two lemmas analogous to Lemma~\ref{lem:cost-to-basis} and \ref{lem:cost-to-smallset} for general $z\ge 1$. Their proofs can be found in Appendix A in \citep{cohenaddad2022towards}. 

\begin{lemma}\label{lem:cost-to-basis-z}
For any even number $k\ge 1$, let $\{c_1,\cdots,c_k\}$ be arbitrary $k$ unit vectors in $\R^d$ such that for each $i$ there exist some $j$ satisfying $c_i=-c_j$. We have
\begin{align*}
    \sum_{i=1}^{d/2} \min_{\ell=1}^k\|e_i-c_{\ell}\|^z \ge 2^{z/2-1}d - 2^{z/2}\max\{1, z/2\}\sqrt{\frac{kd}{2}}.
\end{align*}
\end{lemma}
\begin{lemma}\label{lem:cost-to-smallset-z}
Let $S$ be a set of points in $\R^d$ of size $t$ and $w: S\rightarrow \R^+$ be their weights. For arbitrary $\Delta_p$ for each $p$, there exist $2$ unit vectors $v_1, v_2$ satisfying $v_1=-v_2$, such that
\begin{align*}
    \sum_{p\in S} w(p)\min_{\ell=1,2} \left(\|p-v_{\ell}\|^2+\Delta_p^2 \right)^{z/2} \le &\sum_{s\in P}w(p)(\|p\|^2+1+\Delta_p^2)^{z/2}\\
    &-\min\{1,z/2\}\cdot \frac{2\sum_{p\in S} w(p)(\|p\|^2+1+\Delta_p^2)^{z/2-1} \|p\|}{\sqrt{t}}.
\end{align*}
\end{lemma}

In this proof, the original point set $P$ and three sets of $k$-centers, namely $C_1,C_2,C_3$, are the same as for the case $z=2$. The difference is that now $I=\{j:|S_j|\le \frac{d}{2^z}\}$ and when constructing $C_2$, we use Lemma~\ref{lem:cost-to-smallset-z} in place of Lemma~\ref{lem:cost-to-smallset}. Again, we compare the cost of $P$ and $S$ w.r.t. $C_1,C_2,C_3$ and get the following lemmas.

\begin{lemma}
    For $C_1$ constructed above, we have $\cost(P,C_1) = \frac{kd}{4}\cdot 2^{z/2}$ and 
    \begin{align*}
        \cost(S,C_1) =\sum_{j\in {I}}\sum_{p\in S_j} w(p)(\Delta_p^2+\|\Tilde{p}\|^2 +1)^{z/2} +\sum_{j\in \Bar{I}}\sum_{p\in S_j}w(p)\|p-c_j\|^{z}.
    \end{align*}
\end{lemma}
\begin{proof}
Since $e_i$ is orthogonal to $c_j-jLe_0$ and $c_j-jLe_0$ has unit norm for all $i,j$, it follows that
\begin{align}
\cost(P,C_1) &=
    \sum_{j=1}^{k/2}\sum_{i=1}^{d/2} \min_{c\in C_1}\|jLe_0+e_i-c\|^{2\cdot z/2} = \sum_{j=1}^{k/2} \sum_{i=1}^{d/2} \|jLe_0+e_i -c_j\|^{2\cdot z/2} \nonumber\\
    &=\sum_{j=1}^{k/2}\sum_{i=1}^{d/2}(\|e_i\|^2+\|c_j-jLe_0\|^2-2\langle e_i, c_j-jLe_0 \rangle )^{z/2}\nonumber\\
    &=\frac{kd}{4}\cdot 2^{z/2}.\label{eqn:cost-of-c-z}
\end{align}
On the other hand, the cost of $C_1$ w.r.t.\ $S_j$ is
\begin{align}
    \sum_{p\in S_j} \min_{c\in C_1}w(p)\|p-c\|^{2\cdot z/2} &= \sum_{p\in S_j} w(p)\|p-c_j\|^{2\cdot z/2} = \sum_{p\in S_j} w(p)\|p-jLe_0+ jLe_0-c_j\|^{2\cdot z/2} \nonumber\\
    &= \sum_{p\in S_j}w(p) \left( \|p-jLe_0\|^2 + 1 -2\langle p-jLe_0, jLe_0-c_j \rangle \right)^{z/2}.\label{eqn:cost-of-c-to-S-z}
\end{align}
For $j\in I$, the inner product is $0$, and thus the total cost w.r.t.\ $S$ is 
\begin{align*}
    \cost(S,C_1) = \sum_{j\in {I}}\sum_{p\in S_j} w(p)(\Delta_p^2+\|\Tilde{p}\|^2 +1)^{z/2} + \sum_{j\in \Bar{I}}\sum_{p\in S_j}w(p)\|p-c_j\|^{z},
\end{align*}
which finishes the proof.
\end{proof}
For notational convenience, we define $\kappa := \sum_{j\in \Bar{I}}\sum_{p\in S_j}w(p)\|p-c_j\|^{z}$.
Since $S$ is an $\eps$-coreset of $P$, we have 
\begin{align}\label{eqn:weight-constraints-z}
    \frac{kd}{4}\cdot 2^{z/2} - \frac{\eps kd}{4}\cdot 2^{z/2}  \le \sum_{j\in {I}}\sum_{p\in S_j} w(p)(\Delta_p^2+\|\Tilde{p}\|^2 +1)^{z/2} + \kappa \le \frac{kd}{4}\cdot 2^{z/2} + \frac{\eps kd}{4}2^{z/2}.
\end{align}

Next we consider a different set of $k$ centers denoted by $C_2$. By Lemma~\ref{lem:cost-to-smallset-z}, there exists unit vectors $v^j_1,v^j_2 \in \R^d$ satisfying $v^j_1=-v^j_2$ such that
\begin{align}
    \sum_{p\in S_j} w(p)(\min_{\ell=1,2} \left(\|\Tilde{p}-v^j_{\ell}\|^2+\Delta^2_p\right)^{z/2}) \le&
    \sum_{p\in S_j}w(p)(\|\Tilde{p}\|^2+1 +\Delta^2_p )^{z/2} \nonumber\\
    &-  \min\{1,z/2\}\frac{2\sum_{p\in S_j} w(p)(\|\Tilde{p}\|^2+1 +\Delta^2_p)^{z/2-1} \|\Tilde{p}\|}{\sqrt{|S_j|}}. \label{eqn:small-coreset-cost-z}
\end{align}
Applying this to all $j\in I$ and get corresponding $v^j_1,v^j_2$ for all $j\in I$. Let $C_2=\{u_1^1,u_2^2,\cdots, u_1^{k/2},u_2^{k/2}\}$ be a set of $k$ centers in $\R^{d+1}$ defined as follows: if $j\in I$, $u_{\ell}^j$ is $v_{\ell}^j$ with an additional $0$th coordinate with value $jL$, making them lie in $H_j$; for $j\in \Bar{I}$, we use the same centers as in $C_1$, i.e., $u_{1}^j=u_{2}^j =c_j$. 




\begin{lemma}
    For $C_2$ constructed above, we have 
    \begin{align*}
        \cost(P,C_2) \ge 2^{z/2}\left(\frac{kd}{4} -\max\{1, z/2\}\sqrt{d}|I|\right), \text{ and } 
    \end{align*} 
    \begin{align*}
        \cost(S,C_2) \le& \sum_{j\in I}\sum_{p\in S_j}w(p)(\|\Tilde{p}\|^2+1 +\Delta^2_p )^{z/2} \\
    &-  \min\{1,z/2\}\sum_{j\in I}\frac{2\sum_{p\in S_j} w(p)(\|\Tilde{p}\|^2+1 +\Delta^2_p)^{z/2-1} \|\Tilde{p}\|}{\sqrt{|S_j|}}+\kappa.
    \end{align*}
\end{lemma}
\begin{proof}
By \eqref{eqn:small-coreset-cost-z}, 
\begin{align*}
\cost(S,C_2) &= \sum_{j=1}^{k/2} \sum_{p\in S_j}w(p)\min_{c\in C_2}\|p-c\|^{2\cdot z/2} =
    \sum_{j\in I}\sum_{p\in S_j} w(p)\min_{\ell=1,2} (\|\Tilde{p}-v^j_{\ell}\|^2+\Delta^2_p)^{z/2} +\kappa\\
    &\le 
    \sum_{j\in I}\sum_{p\in S_j}w(p)(\|\Tilde{p}\|^2+1 +\Delta^2_p )^{z/2} \\
    &-  \min\{1,z/2\}\sum_{j\in I}\frac{2\sum_{p\in S_j} w(p)(\|\Tilde{p}\|^2+1 +\Delta^2_p)^{z/2-1} \|\Tilde{p}\|}{\sqrt{|S_j|}}+\kappa.
\end{align*}
By Lemma~\ref{lem:cost-to-basis-z} (with $k=2$), we have
\begin{align*}
    \sum_{i=1}^{d/2} \min_{\ell=1,2}\|e_i-v^j_{\ell}\|^z \ge 2^{z/2-1}d - 2^{z/2}\max\{1, z/2\}\sqrt{d}.
\end{align*}
It follows that
\begin{align*}
    \cost(P,C_2)&=\sum_{j=1}^{k/2}\sum_{i=1}^{d/2} \min_{c\in C_2}\|jLe_0+e_i-c\|^{z} = \sum_{j\in I}\sum_{i=1}^{d/2} \min_{\ell=1,2} \|e_i-v^{j}_{\ell}\|^{2\cdot z/2} + \sum_{j\in \Bar{I}}\sum_{i=1}^{d/2} \|jLe_0+e_i-c_j\|^{2\cdot z/2} \\
    & \ge \left( 2^{z/2-1}d - 2^{z/2}\max\{1, z/2\}\sqrt{d} \right)|I| + |\Bar{I}|\frac{d}{2}\cdot 2^{z/2}= \frac{kd}{4}2^{z/2} - 2^{z/2}\max\{1, z/2\}\sqrt{d}|I|,
\end{align*}
where in the inequality, we also used the orthogonality between $e_i$ and $c_j-jLe_0$.
\end{proof}




Since $S$ is an $\eps$-coreset of $P$, we have
\begin{align*}
    &2^{z/2}\left(\frac{dk}{4}-\max\{1, z/2\}|I|\sqrt{d} - \frac{\eps dk}{4}\right) \le 2^{z/2}\left(\frac{kd}{4} -\max\{1, z/2\}\sqrt{d}|I|\right)(1-\eps) \\
    &\le \sum_{j\in I}\sum_{p\in S_j}w(p)(\|\Tilde{p}\|^2+1 +\Delta^2_p )^{z/2} -  \min\{1,z/2\}\sum_{j\in I}\frac{2\sum_{p\in S_j} w(p)(\|\Tilde{p}\|^2+1 +\Delta^2_p)^{z/2-1} \|\Tilde{p}\|}{\sqrt{|S_j|}}+\kappa,
\end{align*}
which implies
\begin{align}
    &\min\{1,z/2\}\sum_{j\in I}\frac{2\sum_{p\in S_j} w(p)(\|\Tilde{p}\|^2+1 +\Delta^2_p)^{z/2-1} \|\Tilde{p}\|}{\sqrt{|S_j|}}\nonumber\\
    &\le \sum_{j\in I}\sum_{p\in S_j}w(p)(\|\Tilde{p}\|^2+1 +\Delta^2_p )^{z/2} - 2^{z/2}\left(\frac{dk}{4}-\max\{1, z/2\}|I|\sqrt{d} - \frac{\eps dk}{4}\right) + \kappa
    \nonumber\\
    &\le  \frac{kd}{4}\cdot 2^{z/2} + \frac{\eps kd}{4}2^{z/2}  - 2^{z/2}\left(\frac{dk}{4}-\max\{1, z/2\}|I|\sqrt{d} - \frac{\eps dk}{4}\right) \quad\textnormal{by \eqref{eqn:weight-constraints-z}} \nonumber\\
    &= \max\{1, z/2\} |I|\sqrt{d}2^{z/2} +\frac{\eps kd}{2}2^{z/2}. \nonumber
\end{align}
By definition, $|S_j| \le d/t^2$, so
\begin{align*}
      \min\{1,\frac{z}{2}\} \sum_{j\in I} \frac{2\sum_{p\in S_j} w(p)(\|\Tilde{p}\|^2+1 +\Delta^2_p)^{z/2-1} \|\Tilde{p}\|}{\sqrt{d/t^2}}\le \min\{1,\frac{z}{2}\}\sum_{j\in I}\frac{2\sum_{p\in S_j} w(p)(\|\Tilde{p}\|^2+1 +\Delta^2_p)^{z/2-1} \|\Tilde{p}\|}{\sqrt{|S_j|}},
\end{align*}
and it follows that
\begin{align}\label{eqn:size-constraint-z}
     \min\{1,\frac{z}{2}\} \sum_{j\in I} \frac{\sum_{p\in S_j} w(p)(\|\Tilde{p}\|^2+1 +\Delta^2_p)^{z/2-1} \|\Tilde{p}\|}{\sqrt{d}} 
     \le \frac{\max\{1, z/2\} |I|\sqrt{d} 2^{z/2} +\frac{\eps kd}{2}2^{z/2}} {2t}.
\end{align}

Finally we consider a third set of $k$ centers $C_3$. Similarly, there are two centers per group. We set $m$ be a power of $2$ in $[d/2,d]$. Let $h_1,\cdots,h_m$ be the $m$-dimensional Hadamard basis vectors. So all $h_{\ell}$'s are $\{-\frac{1}{\sqrt{m}},\frac{1}{\sqrt{m}}\}$ vectors and $h_1=(\frac{1}{\sqrt{m}},\cdots,\frac{1}{\sqrt{m}})$. We slightly abuse notation and treat each $h_{\ell}$ as a $d$-dimensional vector by concatenating zeros in the end. For each $h_{\ell}$ construct a set of $k$ centers as follows. For each $j\in \Bar{I}$, we still use two copies of $c_j$.  For $j\in I$, the $0$th coordinate of the two centers is $jL$, then we concatenate $h_{\ell}$ and $-h_{\ell}$ respectively to the first and the second centers. 



\begin{lemma}\label{lem:hadamard-cost-z}
     Suppose $C_3$ is constructed based on $h_{\ell}$. Then for all $\ell\in [m]$, we have 
    \begin{align*}
        \cost(P,C_3) \le 2^{z/2}\left( \frac{kd}{4} - \frac{d|I|}{2}\cdot \frac{\min\{1,z/2\}}{\sqrt{m}} \right), \text{ and } 
    \end{align*} 
    \begin{align*}
        \cost(S,C_3) \ge  \sum_{j\in I}\sum_{p\in S_j} w(p)(\|\Tilde{p}\|^2+1 + \Delta_p^2)^{\frac{z}{2}} - 2\max\{1,\frac{z}{2}\} \sum_{j\in I}\sum_{p\in S_j} w(p)\langle \Tilde{p}, h^p_{\ell} \rangle (\|\Tilde{p}\|^2+1 + \Delta_p^2)^{\frac{z}{2}-1}+\kappa.
    \end{align*}
\end{lemma}

\begin{proof}
For $j\in I$, the cost of the two centers w.r.t.\ $P_j$ is
\begin{align*}
    \cost(P_j,C_3) &= \sum_{i=1}^{d/2} \min_{s=-1,+1}\|e_i - s\cdot h_{\ell}\|^z = \sum_{i=1}^{d/2} (2-2\max_{s=-1,+1}\langle h_{\ell},e_i\rangle)^{z/2}= \frac{d}{2}(2-\frac{2}{\sqrt{m}})^{z/2} \\
    &\le \frac{d}{2}\cdot 2^{z/2} \left(1-\frac{\min\{1,z/2\}}{\sqrt{m}}\right).
\end{align*}
For $j\in \Bar{I}$, the cost w.r.t.\ $P_j$ is $\frac{d}{2}\cdot 2^{z/2}$ by \eqref{eqn:cost-of-c-z}.
Thus, the total cost over all subspaces is 
\begin{align*}
\cost(P,C_3) &\le    \frac{d}{2}\cdot2^{z/2} \left(1-\frac{\min\{1,z/2\}}{\sqrt{m}}\right)|I| + \left(\frac{k}{2} -|I| \right)\frac{d}{2}\cdot 2^{z/2} =  2^{z/2}\left( \frac{kd}{4} - \frac{d|I|}{2}\cdot \frac{\min\{1,z/2\}}{\sqrt{m}} \right).
\end{align*} 

On the other hand, for $j\in I$, the cost w.r.t.\ $S_j$ is 
\begin{align*}
    &\sum_{p\in S_j} w(p)(\Delta_p^2+ \min_{s=\{-1,+1\}} \|\Tilde{p}-s\cdot h_{\ell}\|^2)^{z/2} =\sum_{p\in S_j} w(p) (\|\Tilde{p}\|^2+1 + \Delta_p^2 - 2\max_{s=\{-1,+1\}}\langle \Tilde{p}, s\cdot h_{\ell} \rangle)^{z/2}\\
   & =\sum_{p\in S_j} w(p) (\|\Tilde{p}\|^2+1 + \Delta_p^2 - 2\langle \Tilde{p}, h^p_{\ell} \rangle)^{z/2}\\
   &\ge \sum_{p\in S_j} w(p)(\|\Tilde{p}\|^2+1 + \Delta_p^2)^{\frac{z}{2}} - 2\max\{1,\frac{z}{2}\} \sum_{p\in S_j} w(p)\langle \Tilde{p}, h^p_{\ell} \rangle (\|\Tilde{p}\|^2+1 + \Delta_p^2)^{\frac{z}{2}-1}.
\end{align*}
Here $h^p_{\ell} = s^p\cdot h_{\ell}$, where  $s^p=\arg\max_{s=\{-1,+1\}}\langle \Tilde{p}, s\cdot h_{\ell} \rangle$.
For $j\in \Bar{I}$, the total cost w.r.t.\ $S_j$ is $\kappa$. Thus, the total cost w.r.t.\ $S$ is
\begin{align*}
    \cost(S,C_3) \ge \sum_{j\in I}\sum_{p\in S_j} w(p)(\|\Tilde{p}\|^2+1 + \Delta_p^2)^{\frac{z}{2}} - 2\max\{1,\frac{z}{2}\} \sum_{j\in I}\sum_{p\in S_j} w(p)\langle \Tilde{p}, h^p_{\ell} \rangle (\|\Tilde{p}\|^2+1 + \Delta_p^2)^{\frac{z}{2}-1}+\kappa .
\end{align*}
This finishes the proof.
\end{proof}

\begin{corollary}
Let $S$ be a $\eps$-coreset of $P$, and $I =\{j: |S_j|\le d/4\}$. Then 
\begin{align*}
    2\max\{1,\frac{z}{2}\} \sum_{j\in I}\sum_{p\in S_j} w(p)(\|\Tilde{p}\|^2+1 + \Delta_p^2)^{\frac{z}{2}-1} \|\Tilde{p}\| \ge 2^{z/2}\cdot \left( \frac{d|I|}{2}\cdot\min\{1,z/2\} - \frac{\eps kd \sqrt{d}}{2}\right). \\
\end{align*}
\end{corollary}
\begin{proof}
Since $S$ is an $\eps$-coreset, we have by Lemma~\ref{lem:hadamard-cost-z}
\begin{align*}
    &2\max\{1,\frac{z}{2}\} \sum_{j\in I}\sum_{p\in S_j} w(p)\langle \Tilde{p}, h^p_{\ell} \rangle (\|\Tilde{p}\|^2+1 + \Delta_p^2)^{\frac{z}{2}-1} \ge \sum_{j\in I}\sum_{p\in S_j} w(p)(\|\Tilde{p}\|^2+1 + \Delta_p^2)^{\frac{z}{2}} + \kappa \\
    &~~~~ ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ -2^{z/2}\left( \frac{kd}{4} - \frac{d|I|}{2}\cdot \frac{\min\{1,z/2\}}{\sqrt{m}} \right)(1+\eps)\\
    &\ge \frac{kd}{4}\cdot 2^{z/2} - \frac{\eps kd}{4}\cdot 2^{z/2} - 2^{z/2}\left( \frac{kd}{4} - \frac{d|I|}{2}\cdot \frac{\min\{1,z/2\}}{\sqrt{m}} +\frac{\eps kd}{4} \right) \quad\textnormal{by \eqref{eqn:weight-constraints-z}}\\
    &= 2^{z/2}\cdot \frac{d|I|}{2}\cdot \frac{\min\{1,z/2\}}{\sqrt{m}} - \frac{\eps kd}{2}\cdot 2^{z/2}.
\end{align*}
Note that the above inequality holds for all $\ell\in[m]$, then 
$$ 2\max\{1,\frac{z}{2}\} \sum_{\ell=1}^m\sum_{j\in I}\sum_{p\in S_j} w(p)\langle \Tilde{p}, h^p_{\ell} \rangle (\|\Tilde{p}\|^2+1 + \Delta_p^2)^{\frac{z}{2}-1} \ge 2^{z/2}\cdot \left( \frac{d|I|\sqrt{m}}{2}\cdot\min\{1,z/2\} - \frac{\eps kd m}{2}\right).$$

By the Cauchy-Schwartz inequality, 
\begin{align*}
    \sum_{\ell=1}^m\sum_{j\in I}\sum_{p\in S_j} w(p)\langle \Tilde{p}, h^p_{\ell} \rangle (\|\Tilde{p}\|^2+1 + \Delta_p^2)^{\frac{z}{2}-1} &=  \sum_{j\in I}\sum_{p\in S_j} w(p)\langle \Tilde{p}, \sum_{\ell=1}^m h^p_{\ell} \rangle (\|\Tilde{p}\|^2+1 + \Delta_p^2)^{\frac{z}{2}-1}  \\
    &\le \sum_{j\in I}\sum_{p\in S_j} w(p)(\|\Tilde{p}\|^2+1 + \Delta_p^2)^{\frac{z}{2}-1} \|\Tilde{p}\|\cdot  \|\sum_{\ell=1}^m h^p_{\ell}\|   \\
    &= \sqrt{m}\sum_{j\in I}\sum_{p\in S_j} w(p)(\|\Tilde{p}\|^2+1 + \Delta_p^2)^{\frac{z}{2}-1} \|\Tilde{p}\|.
\end{align*}
Therefore, we have
\begin{align*}
    2\max\{1,\frac{z}{2}\} \sum_{j\in I}\sum_{p\in S_j} w(p)(\|\Tilde{p}\|^2+1 + \Delta_p^2)^{\frac{z}{2}-1} \|\Tilde{p}\| &\ge  2^{z/2}\cdot \left( \frac{d|I|}{2}\cdot\min\{1,z/2\} - \frac{\eps kd \sqrt{m}}{2}\right) \\
    &\ge 2^{z/2}\cdot \left( \frac{d|I|}{2}\cdot\min\{1,z/2\} - \frac{\eps kd \sqrt{d}}{2}\right).
\end{align*}
\end{proof}

Combining the above corollary with \eqref{eqn:size-constraint-z}, we have
\begin{align*}
    \frac{\min\{1,z/2\}}{2\max\{1,z/2\}}2^{z/2}\cdot \left( \frac{\sqrt{d}|I|}{2}\cdot\min\{1,z/2\} - \frac{\eps kd }{2}\right) \le \frac{\left( \max\{1, z/2\} |I|\sqrt{d} +\frac{\eps kd}{2}\right)2^{z/2}} {2t},
\end{align*}
which implies that
\begin{align*}
    \left(\frac{\min\{1,(z/2)^2\}}{4\max\{1,(z/2)\}}-\frac{\max\{1,z/2\}}{2t}\right)|I| \le  \frac{\min\{1,(z/2)\}\eps kd}{4\max\{1,(z/2)\}}+ \frac{\eps k\sqrt{d}}{4t}.
\end{align*}
So if we set $t = \frac{4\max\{1,(z/2)^2\}}{\min\{1,(z/2)^2\}}$, then
\begin{align*}
    \frac{\min\{1,(z/2)^2\}}{8\max\{1,(z/2)\}}|I| \le \frac{\min\{1,(z/2)\}\eps k\sqrt{d}}{2\max\{1,(z/2)\}} \implies |I| \le \frac{4\eps k\sqrt{d}}{\min\{1,z/2\}}.
\end{align*}

By the assumption $d\le \frac{\min\{1,(z/2)^2\}}{100\eps^2}$, it holds that $|I| \le \frac{2k}{5}$ or $|\Bar{I}|\ge \frac{k}{2} -\frac{2k}{5}=\frac{k}{10}$. Moreover, since $|S_j|>\frac{d}{t^2}$ for each $j\in \Bar{I}$, we have $|S|>\frac{d}{t^2}\cdot \frac{k}{5} = \frac{kd \min\{1,(z/2)^4\}}{\max\{1,(z/2)^4\}}$.
